The Carbon Content of Intergalactic Gas at z=4.25 and its Evolution Toward z=2.4

This paper presents ionization-corrected measurements of the carbon abundance in intergalactic gas at 4.0 < z < 4.5, using spectra of three bright quasars obtained with the MIKE spectrograph on Magellan. By measuring the CIV strength in a sample of 131 discrete HI-selected quasar absorbers with \rho/\bar{\rho}>1.6, we derive a median carbon abundance of [C/H]=-3.55, with lognormal scatter of approximately ~0.8 dex. This median value is a factor of two to three lower than similar measurements made at z~2.4 using CIV and OVI. The strength of evolution is modestly dependent on the choice of UV background spectrum used to make ionization corrections, although our detection of an abundance evolution is generally robust with respect to this model uncertainty. We present a framework for analyzing the effects of spatial fluctuations in the UV ionizing background at frequencies relevant for CIV production. We also explore the effects of reduced flux between 3-4 Rydbergs (as from HeII Lyman series absorption) on our abundance estimates. At HeII line absorption levels similar to published estimates the effects are very small, although a larger optical depth could reduce the strength of the abundance evolution. Our results imply that ~50% of the heavy elements seen in the IGM at z~2.4 were deposited in the 1.3 Gyr between z~4.3 and z~2.4. The total implied mass flux of carbon into the Lyman alpha forest would constitute ~30% of the IMF-weighted carbon yield from known star forming populations over this period.

==> macros.tex <==
\newcommand{\lya}{Ly-$\alpha$~}
\newcommand{\lyb}{Ly-$\beta$~}
\newcommand{\lyg}{Ly-$\gamma$~}
\newcommand{\lyd}{Ly-$\delta$~}
\newcommand{\nhi}{N_{\mhi}}
\newcommand{\novi}{N_{\movi}}
\newcommand{\nciv}{N_{\mciv}}
\newcommand{\pcmsq}{cm$^{-2}$}
%
\newcommand{\cii}{C~{\sc ii}~}
\newcommand{\ciii}{C~{\sc iii}~}
\newcommand{\civ}{C~{\sc iv}~}
\newcommand{\cv}{C~{\sc v}~}
\newcommand{\cvi}{C~{\sc vi}~}
%
\newcommand{\oi}{O~{\sc i}~}
\newcommand{\ov}{O~{\sc v}~}
\newcommand{\ovi}{O~{\sc vi}~}
\newcommand{\ovii}{O~{\sc vii}~}
\newcommand{\oviii}{O~{\sc viii}~}
%
\newcommand{\siii}{Si~{\sc ii}~}
\newcommand{\siiii}{Si~{\sc iii}~}
\newcommand{\siiv}{Si~{\sc iv}~}
%
\newcommand{\hi}{H~{\sc i}~}
\newcommand{\hii}{H~{\sc ii}~}
%
\newcommand{\heii}{He~{\sc ii}~}
\newcommand{\heiii}{He~{\sc iii}~}
\newcommand{\heiinsp}{He~{\sc ii}}
\newcommand{\heiiinsp}{He~{\sc iii}}
\newcommand{\civnsp}{C~{\sc iv}}
\newcommand{\cvnsp}{C~{\sc v}}
\newcommand{\ovinsp}{O~{\sc vi}}
\newcommand{\hinsp}{H~{\sc i}}
\newcommand{\ciiinsp}{C~{\sc iii}}
\newcommand{\ciinsp}{C~{\sc ii}}
%
\newcommand{\nv}{N~{\sc v}~}
%
\newcommand{\feii}{Fe~{\sc ii}~}
%
\newcommand{\alii}{Al~{\sc ii}~}
\newcommand{\aliii}{Al~{\sc iii}~}
%
\newcommand{\nii}{N~{\sc ii}~}
%
\newcommand{\mgii}{Mg~{\sc ii}~}
%
\newcommand{\oden}{\rho/\bar{\rho}}
\newcommand{\ang}{\AA~}
%
\newcommand{\mhi}{{\rm H \; \mbox{\tiny I}}}
\newcommand{\mov}{{\rm O \; \mbox{\tiny V}}}
\newcommand{\movi}{{\rm O \; \mbox{\tiny VI}}}
\newcommand{\movii}{{\rm O \; \mbox{\tiny VII}}}
\newcommand{\moviii}{{\rm O \; \mbox{\tiny VIII}}}
\newcommand{\mciv}{{\rm C \; \mbox{\tiny IV}}}
\newcommand{\msiiv}{{\rm Si \; \mbox{\tiny IV}}}
\newcommand{\msiii}{{\rm Si \; \mbox{\tiny II}}}
\newcommand{\mcii}{{\rm C \; \mbox{\tiny II}}}
\newcommand{\mciii}{{\rm C \; \mbox{\tiny III}}}
\newcommand{\msiiii}{{\rm Si \; \mbox{\tiny III}}}
\newcommand{\mnii}{{\rm N \; \mbox{\tiny II}}}
\newcommand{\mmgii}{{\rm Mg \; \mbox{\tiny II}}}
\newcommand{\mnv}{{\rm N \; \mbox{\tiny V}}}
\newcommand{\mheii}{{\rm He \; \mbox{\tiny II}}}
\newcommand{\mheiii}{{\rm He \; \mbox{\tiny III}}}
\newcommand{\malii}{{\rm Al \; \mbox{\tiny II}}}
\newcommand{\mfeii}{{\rm Fe \; \mbox{\tiny II}}}
%
\newcommand{\dagnote}{\tablenotemark{\dagger}}
\newcommand{\ddagnote}{\tablenotemark{\dagger\dagger}}
\newcommand{\hinv}{h_{71}^{-1}}
\newcommand{\ha}{H$\alpha$ ~}
\newcommand{\kms}{km s$^{-1}$}

